The Grover search as a naturally occurring phenomenon

We provide first evidence that under certain conditions, 1/2-spin fermions may naturally behave like a Grover search, looking for topological defects in a material. The theoretical framework is that of discrete-time quantum walks (QW), i.e. local unitary matrices that drive the evolution of a single particle on the lattice. Some QW are well-known to recover the $(2+1)$--dimensional Dirac equation in continuum limit, i.e. the free propagation of the 1/2-spin fermion. We study two such Dirac QW, one on the square grid and the other on a triangular grid reminiscent of graphene-like materials. The numerical simulations show that the walker localises around the defects in $O(\sqrt{N})$ steps with probability $O(1/\log{N})$, in line with previous QW search on the grid. The main advantage brought by those of this paper is that they could be implemented as `naturally occurring' freely propagating particles over a surface featuring topological---without the need for a specific oracle step. From a quantum computing perspective, however, this hints at novel applications of QW search : instead of using them to look for `good' solutions within the configuration space of a problem, we could use them to look for topological properties of the entire configuration space.

==> PabMacros.tex <==
\newcommand{\x}{\noindent{\color{blue}xxx}\\}
\newcommand{\xx}[1]{\noindent{\color{blue}#1}\\}
\newcommand{\xxx}[2]{{\color{red}  $<$#2$>$ #1 $<\backslash $#2$>$ }}
\newcommand{\couic}[1]{}
\newcommand{\couicfootnote}[1]{}
\newcommand{\couicefootnote}[1]{}
\newcommand{\couicfootnotemark}{}

%\newcommand{i.e.}{{\em i.e. }}
%\newcommand{e.g.}{{\em e.g. }}
%\newcommand{etc.}{{\em etc. }}
%\newcommand{c.f.}{{\em cf. }}
\newcommand{\eg}{e.g.}
\newcommand{\etc}{etc.}
\newcommand{\ie}{i.e.}

\newcommand{\lra}{\longrightarrow}
\newcommand{\ul}{\underline}
\newcommand{\sub}[1]{\langle #1 \rangle}
\newcommand{\ve}[1]{\mathrm{\textbf{#1}}}

\newcommand{\ket}[1]{| #1 \rangle}
%\newcommand{\bra}[1]{\langle #1 |}
%\newcommand{\braket}[2]{\langle #1 | #2 \rangle}
%\newcommand{\trace}{\textrm{Tr}}

\newcommand{\dom}{\textrm{dom}}
\newcommand{\range}{\textrm{range}}

\newcommand{\Herm}{\textrm{Herm}^+_{d^2}(\mathbb{C})}
\newcommand{\herm}{\textrm{Herm}^+_{d}(\mathbb{C})}
\newcommand{\hermdm}{\textrm{Herm}^+_{dm}(\mathbb{C})}
\newcommand{\hermm}{\textrm{Herm}^+_{m}(\mathbb{C})}

\newcommand{\im}{\mathrm Im}
\newcommand{\ii}{\mathrm i}
\newcommand{\europ}{\textup{\emph{\geneuro}}}
\newcommand{\ad}{\operatorname{ad}}
\newcommand{\Id}{\operatorname{Id}}
%\newcommand{\C}{\mathcal{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Supp}{{\bf\mathcal{S}}}
\newcommand{\pa}[1]{\left(#1\right)}
\newcommand{\acco}[1]{\left\{#1\right\}}
\newcommand{\norme}[1]{\left|\left|#1\right|\right|}

\newcommand{\tzero}{{\overline{0}}}
\newcommand{\size}{\textrm{\texttt{size}}}
\newcommand{\corch}[1]{[#1]}
\newcommand{\val}[1]{[\![#1]\!]}
\newcommand{\llaves}[1]{\{#1\}}
\newcommand{\true}{\mathrm{true}}
\newcommand{\false}{\mathrm{false}}
\newcommand{\type}{\colon\!}
\newcommand{\T}{\mathcal{T}}
%\newcommand{\U}{\mathcal{U}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\LL}{\mathcal{LL}}
\newcommand{\BLL}{\mathcal{BLL}}
\newcommand{\SL}{\ensuremath{\mathcal{SL}}}
\newcommand{\mapLLSL}[1]{\kappa_U({#1})}
\newcommand{\lasf}{\lambda 2^{la}}
\newcommand{\rulesf}{^\triangleleft}
\newcommand{\mapsf}{^\natural}
\newcommand{\Tsf}{\mathbb{T}(\lasf)}


